SuperDepth: Self-Supervised, Super-Resolved Monocular Depth Estimation

Recent techniques in self-supervised monocular depth estimation are approaching the performance of supervised methods, but operate in low resolution only. We show that high resolution is key towards high-fidelity self-supervised monocular depth prediction. Inspired by recent deep learning methods for Single-Image Super-Resolution, we propose a sub-pixel convolutional layer extension for depth super-resolution that accurately synthesizes high-resolution disparities from their corresponding low-resolution convolutional features. In addition, we introduce a differentiable flip-augmentation layer that accurately fuses predictions from the image and its horizontally flipped version, reducing the effect of left and right shadow regions generated in the disparity map due to occlusions. Both contributions provide significant performance gains over the state-of-the-art in self-supervised depth and pose estimation on the public KITTI benchmark. A video of our approach can be found at https://youtu.be/jKNgBeBMx0I.

==> tex/proc-losses.tex <==
\subsection{View Synthesis}
~\cite{jaderberg2015spatial}
\label{sec:view-synthesis}
\begin{align}
  p_s \sim K \hat{T}_{t \to s}  \hat{D}(p_t) K^{-1}p_t
  \label{eq:view-synthesis}
\end{align}

\subsection{Generalization to Multi-View Case}
\label{sec:losses}

\textbf{Photometric Loss via Structural Similarity}


\textbf{Disparity Smoothness Loss}


\textbf{Left-Right Disparity Consistency Loss}
\begin{align}
  \mathcal{L}_{c}(d^L) &= 
  \frac{1}{N} \sum_{uv} | d^L_{uv} - \hat{d}^L_{uv} | \\
  \text{where}~~
  \hat{d}^L_{uv} &= d^L_{uv + d^L_{uv}}
  \label{eq:loss-disp-consistency}
\end{align}

\textbf{Multi-view Map Consistency Loss}

\cite{godard2017unsupervised} uses stereo L-R consistency,
\cite{zhou2017unsupervised} uses monocular multi-view consistency,
\cite{godard2018digging} extends to monocular and stereo consistencies
treated separately.

\begin{itemize}
  \item Generalize beyond stereo left-right pair to multi-view and
    multi-camera setup
  \item Key insight from SLAM community: With an initialized
    local map (per-keyframe 2D-to-3D) photometric error minimization
  \item Generalization of~\cite{godard2017unsupervised} and~\cite{zhou2017unsupervised}
\end{itemize}

We re-write~\ref{eq:loss-photo} and~\ref{eq:loss-disp-consistency}.

New \textit{multi-view photometric loss} becomes: 
\begin{align}
  \mathcal{L}_{MVp} &= 
  \frac{1}{K} \sum_{k\in\mathcal{K}} \mathcal{L}_p (\mathcal{I}^k)\\
  \text{where}~~\mathcal{\hat{I}}^k_{uv} &=
  \text{proj}_{\xi_k}(\mathcal{I}^{1:K}, \mathcal{M})
  \label{eq:loss-mv-photo}
\end{align}

New \textit{multi-view disparity consistency loss} becomes: 
\begin{align}
  \mathcal{L}_{MVc} &= 
  \frac{1}{N} \sum_{k\in\mathcal{K}} \mathcal{L}_c(d^k)\\
  \text{where}~~
  \hat{d}^k_{uv} &= \text{proj}_{\xi_k}(\mathcal{M})
  \label{eq:loss-mv-disp-consistency}
\end{align}


\begin{itemize}
\item Extend to multi-view with local maps
\item Generalization of the left-right consistency loss
\end{itemize}

\textbf{Overall loss}
The overall loss is then defined as the weighted of the individual losses incurred in
the SSIM-based photometric error, disparity smoothness, and the
disparity consistency error. The average loss is computed and averaged
over all batches, views, scales, and pixels. 
\begin{align}
  \mathcal{L}_{MV} &= \mathcal{L}_{MVp} + \lambda_1 \mathcal{L}_s + \lambda_2 \mathcal{L}_{MVc}
  \label{eq:loss-overall}
\end{align}


\begin{itemize}
\item Occlusion-aware Photometric Loss
\end{itemize}



==> tex/results/pose-accuracy.tex <==
% \begin{table*}[h]
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \rowcolors{2}{lightgray}{white}
% \begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}cccccc}
% \toprule
% \textbf{Method} &
% \quad Train\quad &
% \quad Context size (\# frames)\quad &
% \quad GT scale\quad &
% \quad Seq. 09\quad & 
% \quad Seq. 10\quad \\
% \midrule
% ORB-SLAM-M (full)~\cite{murartal2015ORBSLAM}& - & all & Y & 0.014 $\pm$ 0.008 & 0.012 $\pm$ 0.011 \\
% ORB-SLAM-M (short)~\cite{murartal2015ORBSLAM}& - & 5 & Y & 0.064 $\pm$ 0.141 & 0.064 $\pm$ 0.130 \\
% SfMLearner (Zhou et al.~\cite{zhou2017unsupervised})& M & 5 & Y & 0.021 $\pm$ 0.017 & 0.020 $\pm$ 0.015 \\
% %SfMLearner (Zhou et al.~\cite{zhou2017unsupervised})$\dagger$ & M & 5 & Y & 0.016 $\pm$ 0.009 & 0.013 $\pm$ 0.009 \\
% *GeoNet (Yin et al.~\cite{yin2018geonet}) & M & 5 & \todosp{???} & 0.012 $\pm$ 0.007 & 0.012 $\pm$ 0.009 \\
% *Mahjourian et al.~\cite{mahjourian2018unsupervised} & M & 5 & \todosp{???} & 0.013 $\pm$ 0.010 & 0.012 $\pm$ 0.011 \\
% *Godard et al.~\cite{godard2018digging} & M & 3 & \todosp{???} & 0.023 $\pm$ 0.013 & 0.018 $\pm$ 0.014 \\
% *DDVO (Wang et al.~\cite{wang2018learning}) & M & \todosp{???} & \todosp{???} & 0.045 $\pm$ 0.108 & 0.018 $\pm$ 0.014 \\
% \midrule
% \textbf{Ours} & M & 5 & Y & $\ddagger$ & $\ddagger$\\
% \textbf{Ours} & M & 10 & Y & $\ddagger$ & $\ddagger$\\
% \textbf{Ours} & MS & 5 & Y & $\ddagger$ & $\ddagger$\\
% \bottomrule
% \end{tabular*}\\\vspace{1mm}
% }
% \caption{Average Absolute Trajectory Error (ATE) in meters: Analysis of pose accuracy of our system on the KITTI Odometry Split~\cite{geiger2013vision}, Stereo (S), Mono(M), Mono + Stereo (MS). All methods are trained on Seq. 00-08 and evaluated on Seq. 09-10. $\ddagger$ \todosp{to get these numbers we will have to train our method on KITTI odometry 00-08 and evaluate on 09-10}.*\todosp{double check if these numbers are obtained after applying scale from GT.}}
% \label{table:pose-accuracy}
% \vspace{-3mm}
% \end{table*}


\begin{table}[h]
% \centering
{
\small
\setlength{\tabcolsep}{0.3em}
\rowcolors{2}{lightgray}{white}
\begin{tabular*}{\colwidth}{l@{\extracolsep{\fill}}ccc}
\toprule
\textbf{Method} &
\quad Seq. 09\quad & 
\quad Seq. 10\quad \\
\midrule
ORB-SLAM-M (full)~\cite{murartal2015ORBSLAM}&  0.014 $\pm$ 0.008 & 0.012 $\pm$ 0.011 \\
ORB-SLAM-M (short)~\cite{murartal2015ORBSLAM}& 0.064 $\pm$ 0.141 & 0.064 $\pm$ 0.130 \\
SfMLearner (Zhou et al.~\cite{zhou2017unsupervised})& 0.021 $\pm$ 0.017 & 0.020 $\pm$ 0.015 \\
%SfMLearner (Zhou et al.~\cite{zhou2017unsupervised})$\dagger$ & M & 5 & Y & 0.016 $\pm$ 0.009 & 0.013 $\pm$ 0.009 \\
*GeoNet (Yin et al.~\cite{yin2018geonet}) & 0.012 $\pm$ 0.007 & 0.012 $\pm$ 0.009 \\
*Mahjourian et al.~\cite{mahjourian2018unsupervised} & 0.013 $\pm$ 0.010 & 0.012 $\pm$ 0.011 \\
*Godard et al.~\cite{godard2018digging} & 0.023 $\pm$ 0.013 & 0.018 $\pm$ 0.014 \\
*DDVO (Wang et al.~\cite{wang2018learning}) & 0.045 $\pm$ 0.108 & 0.018 $\pm$ 0.014 \\
\midrule
\textbf{Ours - 512x192} & $\ddagger$ & $\ddagger$\\
\textbf{Ours - 1024x384} & $\ddagger$ & $\ddagger$\\
\bottomrule
\end{tabular*}\\\vspace{1mm}
}
\caption{Average Absolute Trajectory Error (ATE) in meters: Analysis of pose accuracy of our system on the KITTI Odometry Split~\cite{geiger2013vision}, Stereo (S), Mono(M), Mono + Stereo (MS). All methods are trained on Seq. 00-08 and evaluated on Seq. 09-10. $\ddagger$ \todosp{to get these numbers we will have to train our method on KITTI odometry 00-08 and evaluate on 09-10}.}
\label{table:pose-accuracy}
\vspace{-3mm}
\end{table}

